Strong Fault-Tolerance for Self-Assembly with Fuzzy Temperature

We consider the problem of fault-tolerance in nanoscale algorithmic self-assembly. We employ a variant of Winfree's abstract Tile Assembly Model (aTAM), the two-handed aTAM, in which square "tiles" -- a model of molecules constructed from DNA for the purpose of engineering self-assembled nanostructures -- aggregate according to specific binding sites of varying strengths, and in which large aggregations of tiles may attach to each other, in contrast to the seeded aTAM, in which tiles aggregate one at a time to a single specially-designated "seed" assembly. We focus on a major cause of errors in tile-based self-assembly: that of unintended growth due to "weak" strength-1 bonds, which if allowed to persist, may be stabilized by subsequent attachment of neighboring tiles in the sense that at least energy 2 is now required to break apart the resulting assembly; i.e., the errant assembly is stable at temperature 2. We study a common self-assembly benchmark problem, that of assembling an n x n square using O(log n) unique tile types, under the two-handed model of self-assembly. Our main result achieves a much stronger notion of fault-tolerance than those achieved previously. Arbitrary strength-1 growth is allowed (i.e., the temperature is "fuzzy" and may drift from 2 to 1 for arbitrarily long); however, any assembly that grows sufficiently to become stable at temperature 2 is guaranteed to assemble at temperature 2 into the correct final assembly of an n x n square. In other words, errors due to insufficient attachment, which is the cause of errors studied in earlier papers on fault-tolerance, are prevented absolutely in our main construction, rather than only with high probability and for sufficiently small structures, as in previous fault-tolerance studies.

==> conclusion.tex <==
\section{Conclusion}
\label{sec-conclusion}

%We have defined the notion of fuzzy temperature fault-tolerance, which defines tile self-assembly systems that are strongly resistant to errors due to insufficient attachments. We have shown that for each natural number $n$ there is a tile assembly system that uniquely assembles an $n \times n$ square using $O(\log n)$ unique tile types that is fuzzy temperature fault-tolerant.

Adleman, Cheng, Goel, and Huang \cite{AdChGoHu01} show that for each $n$ there is a (seeded, single-tile addition, non-fault-tolerant) tile assembly system that uniquely assembles an $n \times n$ square using $O(\log n / \log \log n)$ unique tile types, a bound that was shown asymptotically tight by Rothemund and Winfree \cite{RotWin00}. Since our construction uses $\Theta(\log n)$ tile types, an obvious open question is whether there is a fuzzy temperature fault-tolerant tile assembly system that uses the asymptotically optimal $O(\log n / \log \log n)$ to uniquely assemble an $n \times n$ square.
Previous papers \cite{Adl00,AdlCheGoeHuaWas01,AdChGoHu01} have focused on running time for self-assembled shapes. This is a particularly difficult problem for two-handed assembly. The papers attacking the case of the two-handed model \cite{Adl00,AdlCheGoeHuaWas01} expend much effort to derive the expected assembly time for the much simpler problem of assembling a 1-dimensional $1 \times n$ line from $n$ unique tile types that each encode a different position in the line. It is an open problem, first stated in \cite{Adl00}, to prove upper or lower bounds for the optimal time to assemble a square under the two-handed model. It is also an open problem to derive the expected time to completion for our more complicated construction of a fuzzy temperature fault-tolerant square.

Our construction is ``floppy'': many adjacent tiles in the final square are not connected by glues. One would expect that more strongly connected squares are more physically resilient, and they may also help to enforce the steric protection utilized in our construction, so this floppiness may be a disadvantage. Given the goal of preventing all erroneous temperature-1 growth from stabilizing, it seems unlikely that a \emph{full square} -- a square in which every neighboring pair of tiles interact with positive strength -- could be constructed using a fuzzy temperature fault-tolerant system. But it is conceivable that more elaborate use of synchronization could allow extra ``support substructures'' to be used to make our construction ``more fully connected'', while preserving the fuzzy temperature fault-tolerance.

Additionally, the two-handed aTAM, while more realistic than the seeded single-tile attachment aTAM in the sense that it allows for nucleation without a seed, is perhaps less realistic in another sense. The DNA tiles that the aTAM was originally conceived to model, while ostensibly two-dimensional, are not necessarily confined to the plane. In particular, the steric protection that we employ requires the tiles in the $x$-$y$ plane to stay at position $z=0$. If two mismatching gadgets collide, but one of them ``slides'' over the other by moving its bumps out of the plane into $z > 0$, then this could allow the cooperative strength-1 bonds to connect even between mismatching gadgets. We note that other theoretical papers require the assumption of planar steric hindrance as well \cite{DDFIRSS07,RNaseSODA2010,FuSch09,AKKRS09}, so this potential shortcoming is not unique to our technique.

However, floppiness is not an unbreakable law of physics; it is an artifact of one particular experimental method of using DNA to create self-assembling tiles.
%Our result concerns theoretical self-assembly in general.
It is not necessarily infeasible to construct tiles by another method that stay in the plane, or thicken them along the $z$-axis so that some floppiness is tolerable while still enforcing blocking due to steric protection. There are macro-scale techniques for tile self-assembly that are more sturdy and likely to stay in the plane \cite{BisBurKlaKreMalNapBgu05,Rot00}, as well as nanoscale techniques for creating rigid DNA structures \cite{Tensegrity04,RapidChiral05}. Nonetheless, since a promising current technology for constructing self-assembling molecular tiles is the DNA double-crossover implementation, floppiness is a potential problem, for our construction as well as the other theoretical constructions that utilize planar blocking \cite{DDFIRSS07,RNaseSODA2010,FuSch09,AKKRS09}. It remains an open theoretical problem to design a construction of a fuzzy-temperature fault-tolerant square from $O(\log n)$ tile types that is robust to ``3-D floppiness'', and an open experimental problem to design physical molecular tiles that are inflexible enough to allow the use of programmed steric protection as a reliable design tool.  Another open experimental problem in two-handed tile assembly is to determine, for a given tile implementation, what is the largest size of supertiles that will reliably combine.  While it is clear that single tiles experience enough motion in solution to move into positions necessary to combine to growing assemblies, and most likely that supertiles consisting of small numbers of tiles will also do so, there may be an upper bound on the size of supertiles that reliably attach. Note that this potential limitation would also apply to other two-handed constructions employing arbitrarily large supertiles \cite{AGKS05,DDFIRSS07,AdlCheGoeHuaWas01,Adl00}.





==> fuzzy.tex <==
\section{Fuzzy Temperature Fault-Tolerance}
\label{sec-fuzzy}

In this section we introduce the fuzzy temperature model of fault-tolerance in self-assembly.  The fuzzy temperature assembly model permits rampant temperature $\tau=1$ growth of supertiles under the two-handed assembly model.  We are then interested in what producible temperature $\tau=1$ assemblies become stable at temperature $\tau=2$.  If even a single temperature $\tau=1$ assembly becomes stable at temperature $\tau=2$ and is inconsistent with what can be built in a purely temperature $\tau=2$ assembly model, the system is deemed \emph{error prone}.  On the other hand, if all temperature $\tau=1$ assemblies that are stable at temperature $\tau=2$ have a valid temperature $\tau=2$ path of growth to a supertile that is producible under a pure temperature $\tau=2$ model, then the system is deemed \emph{fuzzy temperature fault-tolerant}.  Put another way, even with arbitrary erroneous strength 1 attachments, a fuzzy temperature fault-tolerant system guarantees that such errors cannot stabilize at temperature 2 unless the stabilized supertile can itself grow into a \emph{correct} temperature $\tau=2$ assembly, which means such an assembly is not really an error.

Formally, for a given initial tile set $T$, we define fuzzy temperature fault-tolerance in terms of the following four sets of supertiles: (1) The \emph{dependably produced} (DP) supertiles are those that can be assembled at temperature $\tau=2$ under the two-handed assembly model.  Formally, DP is the set of all producible supertiles for the two-handed assembly system $(T,2)$; (2) The \emph{dependably terminal} (DT) supertiles are all supertiles in DP that cannot grow any further at temperature $\tau=2$.  Formally, DT is the set of terminal, producible supertiles for the two-handed assembly system $(T,2)$; (3) The \emph{plausibly produced} (PP) supertiles are those that can be assembled at temperature $\tau=1$.  Formally, PP is the set of all producible supertiles for the two-handed assembly system $(T,1)$; and (4) The \emph{plausibly stable} (PS) supertiles are all supertiles in PP that are stable at temperature $\tau=2$.

%\begin{itemize}
%    \item The \emph{dependably produced} (DP) supertiles are those which can be assembled at temperature $\tau=2$ under the two-handed assembly model.  Formally, DP is the set of all producible supertiles for the two-handed assembly system $(T,2)$.
%    \item The \emph{dependably terminal} (DT) supertiles are all supertiles in DP which cannot grow any further at temperature $\tau=2$.  Formally, DT is the set of terminally produced supertiles for the two-handed assembly system $(T,2)$.
%    \item The \emph{plausibly produced} (PP) supertiles are those which can be assembled at temperature $\tau=1$.  Formally, PP is the set of all producible supertiles for the two-handed assembly system $(T,1)$.
%    \item The \emph{plausibly stable} (PS) supertiles are all supertiles in PP that are stable at temperature $\tau=2$.
%\end{itemize}


%TODO: I am a bit worried about the formal definition of fuzzy temperature fault-tolerance. In particular, $PS \implies DT$ means that for every $PS$ supertile, it can grow into something in $DT$, but does not specify that it has to grow into something in $DT$. So it could also potentially grow into something terminal but not producible at temperature 2, unless there is some reason I am missing why that could not be the case. How about if we state that $PS \implies DT$ means: (for all supertiles $\alpha \in PS$) (for all terminal supertiles $\beta$ such that $\alpha \to \beta$), $\beta \in DT$. Then this would mean that \emph{everything} terminal that could be produced from $\alpha$ (not just \emph{something} that could be produced from $\alpha$) is something that could occur anyway.


%Intuitively, DT denotes a final collection of supertiles that can be expected to be built given enough time for assembly in a temperature $2$ system. On the other hand, due to the occasional assembly of supertiles with only strength 1 attachments, elements in PP will (plausibly) be assembled.  Elements of PP that are not stable at temperature $\tau=2$ intuitively will eventually break apart and are not of concern.  However, these assemblies may grow to a point in which they become stable at temperature $\tau=2$, in which case they will not break apart.  Such assemblies constitute the set PS.  The goal is to design a system such that each element of PS can grow into an element of DT at temperature $\tau=2$ (written $PS \Rightarrow DT$), and that DT is the set of desired shapes to be assembled.  Put another way, we want to avoid the design of an error prone system in which stable assemblies that are inconsistent with the desired final assembly are built by erroneous $\tau=1$ strength attachments.

Intuitively, DT denotes a final collection of supertiles that can be expected to be built given enough time for assembly in a temperature $2$ system. On the other hand, due to the occasional assembly of supertiles with only strength 1 attachments, elements in PP will (plausibly) be assembled.  Elements of PP that are not stable at temperature $\tau=2$ intuitively will eventually break apart and are not of concern.  However, these assemblies may grow to a point in which they become stable at temperature $\tau=2$, in which case they will not break apart.  Such assemblies constitute the set PS.  The goal is to design a system such that for each element $\alpha$ of PS, every terminal $\beta$ into which $\alpha$ can grow at temperature $\tau=2$ is an element of DT (written $PS \Rightarrow DT$), and that DT is the set of desired shapes to be assembled.  Put another way, we want to avoid the design of an error prone system in which stable assemblies that are inconsistent with the desired final assembly are built by erroneous $\tau=1$ strength attachments.

More precisely, the fuzzy temperature fault-tolerance design problem is as follows:
\paragraph{\textbf{fuzzy temperature fault-tolerance design problem:}} Given a target shape $\Upsilon$, the goal is to design a tile set such that: (1) $PS \Rightarrow DT$ (fuzzy temperature fault-tolerance constraint); and (2) all supertiles in DT have shape $\Upsilon$. (Desired goal shape is the unique output of the assembly.)

For the remainder of this paper, we attempt to solve the fuzzy temperature fault-tolerance problem for the benchmark example of an $n\times n$ square.  As a metric, we are interested in minimizing the number of distinct tile types required to assemble a square while adhering to the fuzzy temperature fault-tolerance constraint; the problem is trivialized if one allows $n^2$ different tile types to hard-code each position in the square (or even using $O(n)$ tile types to use the non-cooperative ``comb'' structure from \cite{RotWin00}).  We show that a sleek $O(\log n)$ tile complexity is achievable, which is very close to the $O\left(\frac{\log n}{\log\log n}\right)$ bound that can be achieved with no fault-tolerance constraint (in the seeded, single-tile addition model). 

==> intro.tex <==
\section{Introduction}
\label{sec-intro}


Tile-based self-assembly is a model of ``algorithmic crystal growth'' in which square ``tiles'' represent molecules that bind to each other via specific and variable-strength bonds on their four sides, driven by random mixing in solution but constrained by the local binding rules of the tile bonds.  Beginning with the experimental work of Seeman in the early 1980s \cite{Seem82}, such molecules have been engineered from DNA in the laboratory, and used to create a variety of sophisticated self-assembled structures \cite{RoPaWi04,BarSchRotWin09,CheSchGoeWin07,MaoLabReiSee00,WinLiuWenSee98,LiuShaSee99,MaoSunSee99} such as Sierpinski triangles and binary counters.  Erik Winfree \cite{Winf98,Winfree98simulationsof}, based on experimental work of Seeman \cite{Seem82}, modified Wang's mathematical model of tiling \cite{Wang61,Wang63} to add a physically plausible mechanism for growth through time.  Winfree defined two models of tile-based self-assembly, the abstract Tile Assembly Model (aTAM) and the kinetic Tile Assembly Model (kTAM). In both models, the fundamental components are un-rotatable, but
translatable square ``tile types'' whose sides are labeled with glue
``colors'' and ``strengths.'' Two tiles that are placed next to each
other \emph{interact} if the glue colors on their abutting sides
match, and in the aTAM, a tile \emph{binds} to an assembly if it interacts on all sides with total strength at least a certain ambient
``temperature,'' usually taken to be 2.
In particular, if a tile has two strength-1 glues, both of them must match the corresponding glues in the assembly in order to remain bound.

In the more thermodynamically plausible kTAM, tiles may bind even if they interact with strength less than 2, but are assumed to detach at a rate inversely and exponentially proportional to the strength with which they interact. Hence tiles attached with strength 1 detach ``quickly'', and tiles attached with strength 2 detach ``slowly''. A tile attached with only strength 1 (a so-called ``insufficient attachment'') represents a potential error, as its other strength-1 glue may be mismatched with the abutting portion of the assembly, or mismatched with what is eventually intended to be placed at that position. However, since strength-1 attachments are assumed to detach after a short time, an insufficient attachment actualizes into a permanent error only if another tile first binds to secure the faulty tile in place, causing the entire assembly to become stable at temperature 2. That is, by ``wandering'' temporarily through the space of assemblies producible at temperature 1, we may arrive at an assembly not producible at temperature 2, yet that, once formed, is stable at temperature 2. The development of physical and algorithmic mechanisms for preventing such errors remains a formidable challenge in nanoscale self-assembly.

Stated informally, the kTAM refines the aTAM by endowing it with a mechanism for error (temporary binding of tiles with strength 1) as well as a mechanism for error correction (eventual detachment of tiles, even those bound with strength 2). Indeed, numerous papers have used these two mechanisms for high-probability error correction in the kTAM \cite{Winfree98simulationsof,WinBek03,ChenGoel04,ReiSahYin04,CheSchGoeWin07,ChenGL08}.  In each of these papers except \cite{Winfree98simulationsof}, the same basic principle is used to achieve error correction, known as \emph{proofreading}. If an insufficient attachment results in mismatching glues, this error is ``amplified'' by forcing further growth to require many other insufficient attachments to stabilize. Since these happen only slowly, the assembly process is slowed down, giving time for the tiles that stabilized the original insufficient attachment to detach, thus correcting the original error. In \cite{Winfree98simulationsof}, Winfree also shows how errors are removed through the detaching of tiles, although there is no ``error-amplification process''; Winfree shows that by setting the ratio of the forward rate to the reverse rate sufficiently small (thus slowing down the entire assembly process), erroneous tiles will detach with high probability.
Other papers have investigated algorithmic correction of other types of errors \cite{Winfree06,SoloveichikCW08,SchWin04,SchWin07,Luhrs08%,ChenGL08
} and physical, rather than algorithmic, mechanisms for error suppression \cite{ChenEtAl04n,MLR07,FujZhaWinMur09}.

We work in a variant of the aTAM known as the \emph{two-handed} aTAM \cite{AGKS05,DDFIRSS07,Winfree06,Luhrs08,AdlCheGoeHuaWas01,Adl00,RNaseSODA2010}. Winfree's original model, the \emph{seeded} aTAM \cite{Winf98,Winfree98simulationsof}, stipulates that assembly begins from a specially-designated ``seed'' tile type, and all binding events consist of the attachment of a single tile to the growing assembly that contains the seed. The seed thus serves as a \emph{nucleation point} from which all further growth occurs. In reality, such single-point nucleation is difficult to enforce \cite{SchWin07,SchWin04} as tiles with matching glues may attach to each other in solution, even if neither of them is connected to the seed tile.  The two-handed aTAM models this sort of growth by dispensing with the idea of a seed, and simply defining an assembly to be producible if 1) it consists of a single tile (base case), or 2) it results from the stable aggregation of two producible assemblies (recursive case). We emphasize that the present paper does not introduce this two-handed version of the model; it has been studied by numerous authors \cite{AGKS05,DDFIRSS07,Winfree06,Luhrs08,AdlCheGoeHuaWas01,Adl00,RNaseSODA2010} under various names, such as the ``multiple tile'' model or the ``polyomino'' model.

Not only is the two-handed aTAM a more realistic model in the sense of accounting for unseeded nucleation, it allows us to use the geometry of partially-formed assemblies, rather than relying solely on (error-prone) glue specificity, to enforce binding rules between subassemblies. This phenomenon, geometric blocking that prevents bond formation, is well-studied in chemistry and is known as \emph{steric hindrance} \cite[Section 5.11]{WadeOrganicChemistry91} or, particularly when employed as a design tool for intentional prevention of unwanted binding in synthesized molecules, \emph{steric protection} \cite{HellerPugh1,HellerPugh2,GotEtAl00}. Using the mechanism of steric protection, we are able to achieve a much stronger notion of fault-tolerance than that described in previous error-correction papers. Informally, our model of fault-tolerance, which we term the \emph{fuzzy temperature} model, is as follows (a formal description is given in Section \ref{sec-fuzzy}). Similarly to the kTAM, we allow strength-1 insufficient attachments to occur. However, we do not model forward or reverse rates of growth as in the kTAM, as there is no need to employ the higher reverse rates of insufficient attachments: any insufficient attachments that lead to an assembly that is stable at temperature 2 \emph{were never errors in the first place}, as such an assembly can always lead to an assembly that was producible with only strength-2 growth. That is, viewed as a modification of the aTAM, we allow the temperature to be ``fuzzy'', occasionally drifting from 2 down to 1, which allows strength-1 growth for as long as the temperature remains low. However, once the temperature is raised back to 2, thus dissolving any structure that is stable only at temperature 1, the stable assemblies that are left over are all assemblies that are already producible at temperature 2 or that can grow into a temperature-2-producible assembly. Therefore, while insufficient attachments can occur, errors due to insufficient attachments cannot occur, since temperature-2 stabilization of such errors, which our construction prevents, is required for the errors to become permanent.

We focus on the problem of assembling an $n \times n$ square, a common benchmark problem for demonstrating the use of self-assembly techniques \cite{RotWin00,KaoSchS08,RSAES,BeckerRR06,AdChGoHu01,AGKS05,KS07}. In particular, our main result is the construction of a tile set with $O(\log n)$ unique tile types (which is close to the $\Omega(\log n / \log \log n)$ optimal lower bound \cite{RotWin00}) that uniquely assembles into an $n \times n$ square in the two-handed aTAM at temperature 2, and that has the fuzzy-temperature fault-tolerance property described above. In keeping with the ``wandering'' analogy from the beginning of this section, our construction allows arbitrary wandering in the space of assemblies producible at temperature 1, but funnels all such wandering towards a single unique terminal assembly, or towards the oblivion of destruction at temperature 2.\footnote{We emphasize that this is \emph{not} the same as saying that our construction assembles an $n \times n$ square at temperature 1: at temperature 1, many different terminal assemblies can nondeterministically form, most of which are junk. Our construction ensures that when the temperature is raised to 2, all the junk dissolves away, leaving only assemblies that are required to assemble the square, and which could have grown anyway had the temperature remained at 2. In fact, it is an open problem, first stated by Winfree and Rothemund in \cite{RotWin00}, to uniquely assemble an $n \times n$ square at temperature 1 using fewer than $2n - 1$ tile types (compared to our use of $O(\log n)$ tile types). Rothemund and Winfree conjectured that $2n-1$ is a strict lower bound for this problem.}

%TODO: Robbie, I added the next paragraph in response to an email you sent but I am honestly not sure about it since I do not understand thermodynamics very well. How certain are you of this physical interpretation, that our construction allows arbitrarily high forward rates compared to reverse rates? If you are not certain I suggest leaving it out because I don't want Winfree or someone to be a reviewer and tell the PC that we don't understand what we are modeling. (\emph{i.e.,} I would rather hide the fact that I don't understand it)

%Since previous error-correction schemes rely on waiting for the detachment of tiles bound with strength 2 (a time-consuming process by design), such schemes necessarily slow down the assembly process. Our scheme requires no such slowdown; in principle, the ratio of forward to reverse rates -- which governs the net speed at which assembly proceeds -- may be made arbitrarily high. While this may imply that many intermediate assemblies spend a lot of time ``trying out'' erroneous strength-1 growth, our design ensures that none of these can reach a stable state unless they constitute the intended strength-2 growth.


This paper is organized as follows.
Section \ref{sec-tam-informal} gives an informal description of the two-handed aTAM.
\opt{normal,stocsubmission}{Section \ref{sec-tam} formally defines the two-handed aTAM.}
Section \ref{sec-counter} shows a construction of a non-fault-tolerant counter, to introduce some of the main ideas of the full construction.
Section \ref{sec-fuzzy} defines the fuzzy temperature model of fault-tolerance. Section \ref{sec-square-overview} describes a high-level overview of the main construction and explains the basic techniques employed.
\opt{normal,stocsubmission}{
    Section \ref{sec-square} explains the main construction in detail.
%    Section \ref{sec-runtime} defines a model of running time for two-handed assembly and derives a running time for our construction.
}
Section \ref{sec-conclusion} concludes the paper and states open questions.




==> tam-informal.tex <==
\section{Informal Description of the Two-Handed Abstract Tile Assembly Model}
\label{sec-tam-informal}

This section gives a brief informal sketch of the two-handed temperature-2 abstract Tile Assembly Model (aTAM).
\opt{stocsubmission}{The model is described formally, and more generally, in Section \ref{sec-tam}.}

A \emph{tile type} is a unit square with four sides, each having a \emph{glue} consisting of a \emph{label} (a finite string) and \emph{strength} (0, 1, or 2).
We assume a finite set $T$ of tile types, but an infinite number of copies of each tile type, each copy referred to as a \emph{tile}. A \emph{supertile}
%[DSD: e.g. means "for example"; a.k.a. means "also known as"; they are not synonyms]
%(e.g., \emph{assembly})
(a.k.a., \emph{assembly})
is a positioning of tiles on the integer lattice $\Z^2$.
Two adjacent tiles in a supertile \emph{interact} if the glues on their abutting sides are equal and have positive strength.
Each supertile induces a \emph{binding graph}, a grid graph whose vertices are tiles, with an edge between two tiles if they interact.
The supertile is \emph{$\tau$-stable} if every cut of its binding graph has strength at least $\tau$, where the weight of an edge is the strength of the glue it represents.
That is, the supertile is stable if at least energy $\tau$ is required to separate the supertile into two parts.
A \emph{tile assembly system} (TAS) is a pair $\calT = (T,\tau)$, where $T$ is a finite tile set and $\tau$ is the \emph{temperature}, usually 1 or 2.
Given a TAS $\calT=(T,\tau)$, a supertile is \emph{producible} if either it is a single tile from $T$, or it is the $\tau$-stable result of translating two producible assemblies.
A supertile $\alpha$ is \emph{terminal} if for every producible supertile $\beta$, $\alpha$ and $\beta$ cannot be $\tau$-stably attached.
A TAS is \emph{directed} (a.k.a., \emph{deterministic}, \emph{confluent}) if it has only one terminal, producible supertile.
Given a connected shape $X \subseteq \Z^2$,  a TAS $\calT$ \emph{produces $X$ uniquely} if every producible, terminal supertile places tiles only on positions in $X$ (appropriately translated if necessary).



==> tam.tex <==
\clearpage

\newcommand{\ress}[1]{\mathrm{res}_\mathrm{st}[ #1 ]}
\newcommand{\prodstate}[1]{\mathcal{S}[ #1 ]}
\newcommand{\termstate}[1]{\mathcal{S}_{\Box}[ #1 ]}
\renewcommand{\succ}{\mathrm{succ}}

\section{Two-Handed Abstract Tile Assembly Model}
\label{sec-tam}

In this section we formally define a variant of Erik Winfree's abstract Tile Assembly Model \cite{Winf98,Winfree98simulationsof} modified to model unseeded growth, known as the \emph{two-handed} aTAM, which has been studied previously under various names \cite{AGKS05,DDFIRSS07,Winfree06,Luhrs08,AdlCheGoeHuaWas01,Adl00}. In the two-handed aTAM, any two assemblies can attach to each other, rather than enforcing that tiles can only accrete one at a time to an existing seed assembly. In this section we define the model to allow for infinite assemblies and systems that produce more than one terminal assembly, even though our main construction does not have these properties. We also allow for systems that start with a finite number of tile types, even though the description of our main construction is in terms of an infinite supply of tiles.

$\lg(x)$ and $\log(x)$ each denote the base-2 logarithm of $x$, and $\ln(x)$ denotes the base-$e$ logarithm of $x$. We work in the $2$-dimensional discrete space $\Z^2$. Define the set
$U_2 = \{(0,1), (1,0), (0,-1), (-1,0)\}$ to be the set of all
\emph{unit vectors}, i.e., vectors of length 1 in $\mathbb{Z}^2$.
All \emph{graphs} in this paper are undirected.
A \emph{grid graph} is a graph $G =
(V,E)$ in which $V \subseteq \Z^2$ and every edge
$\{\vec{a},\vec{b}\} \in E$ has the property that $\vec{a} - \vec{b} \in U_2$.

Intuitively, a tile type $t$ is a unit square that can be
translated, but not rotated, having a well-defined ``side
$\vec{u}$'' for each $\vec{u} \in U_2$. Each side $\vec{u}$ of $t$
has a ``glue'' with ``label'' $\textmd{label}_t(\vec{u})$ -- a string
over some fixed alphabet -- and ``strength''
$\textmd{str}_t(\vec{u})$ -- a nonnegative integer -- specified by its type
$t$. Two tiles $t$ and $t'$ that are placed at the points $\vec{a}$
and $\vec{a}+\vec{u}$ respectively, \emph{bind} with \emph{strength}
$\textmd{str}_t\left(\vec{u}\right)$ if and only if
$\left(\textmd{label}_t\left(\vec{u}\right),\textmd{str}_t\left(\vec{u}\right)\right)
=
\left(\textmd{label}_{t'}\left(-\vec{u}\right),\textmd{str}_{t'}\left(-\vec{u}\right)\right)$.

In the subsequent definitions, given two partial functions $f,g$, we write $f(x) = g(x)$ if~$f$ and~$g$ are both defined and equal on~$x$, or if~$f$ and~$g$ are both undefined on $x$.

Throughout this section, fix a finite set $T$ of tile types.
An \emph{assembly} is a partial
function $\pfunc{\alpha}{\Z^2}{T}$ defined on at least one input, with points $\vec{x}\in\Z^2$ at
which $\alpha(\vec{x})$ is undefined interpreted to be empty space,
so that $\dom \alpha$ is the set of points with tiles.
We write $|\alpha|$ to denote $|\dom \alpha|$, and we say $\alpha$ is
\emph{finite} if $|\alpha|$ is finite. For assemblies $\alpha$
and $\alpha'$, we say that $\alpha$ is a \emph{subassembly} of
$\alpha'$, and write $\alpha \sqsubseteq \alpha'$, if $\dom \alpha
\subseteq \dom \alpha'$ and $\alpha(\vec{x}) = \alpha'(\vec{x})$ for
all $x \in \dom \alpha$.
Two assemblies $\alpha$ and $\beta$ are \emph{disjoint} if $\dom \alpha \cap \dom \beta = \emptyset.$
For two assemblies $\alpha$ and $\beta$, define the \emph{union} $\alpha \cup \beta$ to be the assembly defined for all $\vec{x}\in\Z^2$ by $(\alpha \cup \beta)(\vec{x}) = \alpha(\vec{x})$ if $\alpha(\vec{x})$ is defined, and $(\alpha \cup \beta)(\vec{x}) = \beta(\vec{x})$ otherwise. Say that this union is \emph{disjoint} if $\alpha$ and $\beta$ are disjoint.

The \emph{binding graph of} an assembly $\alpha$ is the grid graph
$G_\alpha = (V, E )$, where $V =
\dom{\alpha}$, and $\{\vec{m}, \vec{n}\} \in E$ if and only if (1)
$\vec{m} - \vec{n} \in U_2$, (2)
$\lab_{\alpha(\vec{m})}\left(\vec{n} - \vec{m}\right) =
\lab_{\alpha(\vec{n})}\left(\vec{m} - \vec{n}\right)$, and (3)
$\strength_{\alpha(\vec{m})}\left(\vec{n} -\vec{m}\right) > 0$.
Given $\tau \in \mathbb{N}$, an
assembly is $\tau$-\emph{stable} (or simply \emph{stable} if $\tau$ is understood from context), if it
cannot be broken up into smaller assemblies without breaking bonds
of total strength at least $\tau$; i.e., if every cut of $G_\alpha$
has weight at least $\tau$, where the weight of an edge is the strength of the glue it represents. In contrast to the model of Wang tiling, the nonnegativity of the strength function implies that glue mismatches between adjacent tiles do not prevent a tile from binding to an assembly, so long as sufficient binding strength is received from the (other) sides of the tile at which the glues match.

%
%The \emph{frontier} of an assembly $\alpha$, written as $\partial
%\alpha$, is the set of locations at which a single tile could be
%added to $\alpha$, while maintaining the $\tau$-stability of
%$\alpha$.

The two-handed aTAM \cite{AGKS05,DDFIRSS07} allows for two assemblies, both possibly consisting of more than one tile, to attach to each other, in contrast to the seeded aTAM \cite{Winfree98simulationsof,RotWin00} in which one of the attaching objects is assumed to be a single tile, and the other is the assembly containing the unique ``seed tile''. Since we must allow that the assemblies might require translation before they can bind, we define a \emph{supertile} to be the set of all translations of a $\tau$-stable assembly, and speak of the attachment of supertiles to each other, modeling that the assemblies attach, if possible, after appropriate translation.

Formally, for assemblies $\alpha,\beta:\Z^2 \dashrightarrow T$ and $\vec{u} \in \Z^2$, we write $\alpha+\vec{u}$ to denote the assembly defined for all $\vec{x}\in\Z^2$ by $(\alpha+\vec{u})(\vec{x}) = \alpha(\vec{x}-\vec{u})$, and write $\alpha \simeq \beta$ if there exists $\vec{u}$ such that $\alpha + \vec{u} = \beta$; i.e., if $\alpha$ is a translation of $\beta$.
Define the \emph{supertile} of $\alpha$ to be the set $\ta = \setr{\beta}{\alpha \simeq \beta}.$
A supertile $\ta$ is \emph{$\tau$-stable} (or simply \emph{stable}) if all of the assemblies it contains are $\tau$-stable; equivalently, $\ta$ is stable if it contains a stable assembly, since translation preserves the property of stability. Note also that the notation $|\ta| \equiv |\alpha|$ is well-defined, since translation preserves cardinality (and note in particular that even though we define $\ta$ as a set, $|\ta|$ does not denote the cardinality of this set, which is always $\aleph_0$).

For two supertiles $\ta$ and $\tb$, and temperature $\tau\in\N$, define the \emph{combination} set $C^\tau_{\ta,\tb}$ to be the set of all supertiles $\tg$ such that there exist $\alpha \in \ta$ and $\beta \in \tb$ such that (1) $\alpha$ and $\beta$ are disjoint, (2) $\gamma \equiv \alpha \cup \beta$ is $\tau$-stable, and (3) $\gamma \in \tg$. That is, $C^\tau_{\ta,\tb}$ is the set of all $\tau$-stable supertiles that can be obtained by attaching $\ta$ to $\tb$ stably, with $|C^\tau_{\ta,\tb}| > 1$ if there is more than one position at which $\beta$ could attach stably to $\alpha$.

It is common with seeded assembly to stipulate an infinite number of copies of each tile, but our definition allows for a finite number of tiles as well. Our definition also allows for the growth of infinite assemblies and finite assemblies to be captured by a single definition, similar to the definitions of \cite{SSADST} for seeded assembly.

Given a set of tiles $T$, define a \emph{state} $S$ of $T$ to be a multiset of supertiles, or equivalently, $S$ is a function mapping supertiles of $T$ to $\N \cup \{\infty\}$, indicating the multiplicity of each supertile in the state. We therefore write $\ta \in S$ if and only if $S(\ta) > 0$.

A \emph{(two-handed) tile assembly system} (\emph{TAS}) is an ordered triple $\mathcal{T} = (T, S, \tau)$, where $T$ is a finite set of tile types, $S$ is the \emph{initial state}, and $\tau\in\N$ is the temperature. Subsequently we assume that $\tau = 2$, unless explicitly stated otherwise. If not stated otherwise, assume that the initial state $S$ is defined $S(\ta) = \infty$ for all supertiles $\ta$ such that $|\ta|=1$, and $S(\tb) = 0$ for all other supertiles $\tb$. That is, $S$ is the state consisting of a countably infinite number of copies of each individual tile type from $T$, and no other supertiles. In such a case we write $\calT = (T,\tau)$ to indicate that $\calT$ uses the default initial state.


Given a TAS $\calT=(T,S,\tau)$, define an \emph{assembly sequence} of $\calT$ to be a sequence of states $\vec{S} = (S_i \mid 0 \leq i < k)$ (where $k = \infty$ if $\vec{S}$ is an infinite assembly sequence), and $S_{i+1}$ is constrained based on $S_i$ in the following way: There exist supertiles $\ta,\tb,\tg$ such that (1) $\tg \in C^\tau_{\ta,\tb}$, (2) $S_{i+1}(\tg) = S_{i}(\tg) + 1$,\footnote{with the convention that $\infty = \infty + 1 = \infty - 1$} (3) if $\ta \neq \tb$, then $S_{i+1}(\ta) = S_{i}(\ta) - 1$, $S_{i+1}(\tb) = S_{i}(\tb) - 1$, otherwise if $\ta = \tb$, then $S_{i+1}(\ta) = S_{i}(\ta) - 2$, and (4) $S_{i+1}(\tilde{\omega}) = S_{i}(\tilde{\omega})$ for all $\tilde{\omega} \not\in \{\ta,\tb,\tg\}$.
That is, $S_{i+1}$ is obtained from $S_i$ by picking two supertiles from $S_i$ that can attach to each other, and attaching them, thereby decreasing the count of the two reactant supertiles and increasing the count of the product supertile. If $S_0 = S$, we say that $\vec{S}$ is \emph{nascent}.

%Unlike the seeded model, an infinite assembly sequence in the two-handed model may not have a unique limit state. For example, consider an assembly sequence that starts from an infinite number of single tiles, then continually creates a size-2 supertile $\ta$ from tiles before attaching $\ta$ to a larger and ever-growing supertile. The count of $\ta$ forever oscillates between 0 and 1, so there is no limit state, although the larger supertile, which is more precisely a sequence of supertiles, will have a well-defined limit.
%
%The \emph{resulting state} of a finite assembly sequence $\vec{S} = (S_i \mid 0 \leq i < k)$ is the state $\ress{\vec{S}} = S_k$. If $\vec{S}$ is infinite and $\lim\limits_{i\to\infty} S_i$ exists, then define $\ress{\vec{S}} = \lim\limits_{i\to\infty} S_i$.
%
%Given two states $S$ and $S'$ of $\calT$, write $S \to_\calT S'$, or simply $S \to S'$ if $\calT$ is clear from context, if there is an assembly sequence $\vec{S} = (S_i \mid 0 \leq i < k)$ such that $S_0 = S$ and $\ress{\vec{S}} = S'$. In this case we say that $S$ \emph{produces} $S'$. It is straightforward to show that $\to_\calT$ is a reflexive, transitive relation on states of $\calT$.
%
%If $S$ is a state such that $(S \to S') \implies (S = S')$, then we say that $S$ is \emph{terminal}. Define $\prodstate{\calT}$ to be the set of all resulting states of nascent assembly sequences of $\calT$, known as the \emph{producible states} of $\calT$. Define $\termstate{\calT} \subseteq \prodstate{\calT}$ to be the set of terminal producible states of $\calT$. $\calT$ is \emph{state-directed} (a.k.a., \emph{state-deterministic}, \emph{state-confluent}) if $|\termstate{\calT}| = 1$.

Given an assembly sequence $\vec{S} = (S_i \mid 0 \leq i < k)$ of $\calT=(T,S,\tau)$ and a supertile $\tg \in S_i$ for some $i$, define the \emph{predecessors} of $\tg$ in $\vec{S}$ to be the multiset $\pred_{\vec{S}}(\tg) = \{\ta,\tb\}$ if $\ta,\tb \in S_{i-1}$ and $\ta$ and $\tb$ attached to create $\tg$ at step $i$ of the assembly sequence, and define $\pred_{\vec{S}}(\tg) = \{ \tg \}$ otherwise. Define the \emph{successor} of $\tg$ in $\vec{S}$ to be $\succ_{\vec{S}}(\tg)=\ta$ if $\tg$ is a predecessor of $\ta$ in $\vec{S}$, and define $\succ_{\vec{S}}(\tg)=\tg$ otherwise. A sequence of supertiles $\vec{\ta} = (\ta_i \mid 0 \leq i < k)$ is a \emph{supertile assembly sequence} of $\calT$ if there is an assembly sequence $\vec{S} = (S_i \mid 0 \leq i < k)$ of $\calT$ such that, for all $1 \leq i < k$, $\succ_{\vec{S}}(\ta_{i-1}) = \ta_i$, and $\vec{\ta}$ is \emph{nascent} if $\vec{S}$ is nascent.

The \emph{result} of a supertile assembly sequence $\vec{\ta}$ is the unique supertile $\res{\vec{\ta}}$ such that there exist an assembly $\alpha \in \res{\vec{\ta}}$ and, for each $0 \leq i < k$, assemblies $\alpha_i \in \ta_i$ such that $\dom{\alpha} = \bigcup_{0 \leq i < k}{\dom{\alpha_i}}$ and, for each $0 \leq i < k$, $\alpha_i \sqsubseteq \alpha$. For all supertiles $\ta,\tb$, we write $\ta \to_\calT \tb$ (or $\ta \to \tb$ when $\calT$ is clear from context) to denote that there is a supertile assembly sequence $\vec{\ta} = ( \ta_i \mid 0 \leq i < k )$ such that $\ta_0 = \ta$ and $\res{\vec{\ta}} = \tb$. It can be shown using the techniques of \cite{Roth01} for seeded systems that for all two-handed tile assembly systems $\calT$ supplying an infinite number of each tile type, $\to_\calT$ is a transitive, reflexive relation on supertiles of $\calT$.

A supertile $\ta$ is \emph{producible}, and we write $\ta \in \prodasm{\calT}$, if it is the result of a nascent supertile assembly sequence. A supertile $\ta$ is \emph{terminal} if, for all producible supertiles $\tb$, $C^\tau_{\ta,\tb} = \emptyset$.\footnote{Note that a supertile $\ta$ could be non-terminal in the sense that there is a producible supertile $\tb$ such that $C^\tau_{\ta,\tb} \neq \emptyset$, yet it may not be possible to produce $\ta$ and $\tb$ simultaneously if some tile types are given finite initial counts, implying that $\ta$ cannot be ``grown'' despite being non-terminal. If the count of each tile type in the initial state is $\infty$, then all producible supertiles are producible from any state, and the concept of terminal becomes synonymous with ``not able to grow'', since it would always be possible to use the abundant supply of tiles to assemble $\tb$ alongside $\ta$ and then attach them.} Define $\termasm{\calT} \subseteq \prodasm{\calT}$ to be the set of terminal and producible supertiles of $\calT$. $\calT$ is \emph{directed} (a.k.a., \emph{deterministic}, \emph{confluent}) if $|\termasm{\calT}| = 1$.

Let $X \subseteq \Z^2$ be a shape. We say $X$ \emph{strictly self-assembles} in $\calT$ if, for all $\ta \in \termasm{\calT}$, there exists $\alpha \in \ta$ such that $\dom \alpha = X$; i.e., $\calT$ uniquely assembles into the shape $X$.

